Physical Passive Patch Adversarial Attacks on Visual Odometry Systems

Deep neural networks are known to be susceptible to adversarial perturbations -- small perturbations that alter the output of the network and exist under strict norm limitations. While such perturbations are usually discussed as tailored to a specific input, a universal perturbation can be constructed to alter the model's output on a set of inputs. Universal perturbations present a more realistic case of adversarial attacks, as awareness of the model's exact input is not required. In addition, the universal attack setting raises the subject of generalization to unseen data, where given a set of inputs, the universal perturbations aim to alter the model's output on out-of-sample data. In this work, we study physical passive patch adversarial attacks on visual odometry-based autonomous navigation systems. A visual odometry system aims to infer the relative camera motion between two corresponding viewpoints, and is frequently used by vision-based autonomous navigation systems to estimate their state. For such navigation systems, a patch adversarial perturbation poses a severe security issue, as it can be used to mislead a system onto some collision course. To the best of our knowledge, we show for the first time that the error margin of a visual odometry model can be significantly increased by deploying patch adversarial attacks in the scene. We provide evaluation on synthetic closed-loop drone navigation data and demonstrate that a comparable vulnerability exists in real data. A reference implementation of the proposed method and the reported experiments is provided at https://github.com/patchadversarialattacks/patchadversarialattacks.

==> sections/020_related.tex <==
\section{Related work}
\label{sec:related}



==> visualizations/fig_alg.tex <==
\begin{minipage}{0.48\linewidth}
\begin{algorithm}[H]
	\caption{Non-universal PGD adversarial attack}
	\label{alg:attack}
	\hspace*{\algorithmicindent} \textbf{Input} $VO$: VO model\\
	\hspace*{\algorithmicindent} \textbf{Input} $A$: Adversarial patch perturbation\\
	\hspace*{\algorithmicindent} \textbf{Input} $x$: trajectory to attack\\
	\hspace*{\algorithmicindent} \textbf{Input} $y$: trajectory ground truth motions\\
	\hspace*{\algorithmicindent} \textbf{Input} $\ell_{train}$: train loss function\\
	\hspace*{\algorithmicindent} \textbf{Input} $\ell_{eval}$: evaluation loss function\\
	\hspace*{\algorithmicindent} \textbf{Input} $\alpha$: step size for the attack\\
	\begin{algorithmic}[1]
		\State $P \leftarrow \text{Uniform}(0, 1)$
		\State $P_\text{best} \leftarrow P$
		\State $\text{Loss}_\text{best} \leftarrow 0$
		\For{$k=1$ to $K$}
            \State \underline{\textbf{optimization step: }}
            \State $\hat{y} \leftarrow VO(A(x,P))$
            \State $g \leftarrow \nabla_{P} \ell_{train}(\hat{y}, y)$
            \State $P \leftarrow P + \alpha \cdot \text{sign}(g)$
            \State $P \leftarrow clip(P,0,1)$
            \State \underline{\textbf{evaluate patch: }}
            \State $\hat{y} \leftarrow VO(A(x,P))$
            \State $\text{Loss} \leftarrow \ell_{eval}(\hat{y}, y)$
	        \If{$\text{Loss} > \text{Loss}_\text{best}$}
                \State $P_\text{best} \leftarrow P$
                \State $\text{Loss}_\text{best} \leftarrow \text{Loss}$
	        \EndIf
    	\EndFor
		\State \textbf{return} $P_\text{best}$ 
	\end{algorithmic}
\end{algorithm}
\end{minipage}
\begin{minipage}{0.48\linewidth}
\begin{algorithm}[H]
	\caption{Universal PGD adversarial attack}
	\label{alg:universal_attack}
	\hspace*{\algorithmicindent} \textbf{Input} $VO$: VO model\\
	\hspace*{\algorithmicindent} \textbf{Input} $A$: Adversarial patch perturbation\\
	\hspace*{\algorithmicindent} \textbf{Input} $X_{train}$: Training trajectories\\
	\hspace*{\algorithmicindent} \textbf{Input} $Y_{train}$: Training trajectories ground truth motions\\
	\hspace*{\algorithmicindent} \textbf{Input} $X_{eval}$: eval trajectories\\
	\hspace*{\algorithmicindent} \textbf{Input} $Y_{eval}$: eval trajectories ground truth motions\\
	\hspace*{\algorithmicindent} \textbf{Input} $\ell_{train}$: train loss function\\
	\hspace*{\algorithmicindent} \textbf{Input} $\ell_{eval}$: evaluation loss function\\
	\hspace*{\algorithmicindent} \textbf{Input} $N_{train}$: Number of train trajectories\\
	\hspace*{\algorithmicindent} \textbf{Input} $N_{eval}$: Number of eval trajectories\\
	\hspace*{\algorithmicindent} \textbf{Input} $\alpha$: step size for the attack\\
	\begin{algorithmic}[1]
		\State $P \leftarrow \text{Uniform}(0, 1)$
		\State $P_\text{best} \leftarrow P$
		\State $\text{Loss}_\text{best} \leftarrow 0$
		\For{$k=1$ to $K$}
            \State \underline{\textbf{optimization step: }}
            \State $g \leftarrow 0$
	        \For{$i=1$ to $N_{train}$}
                \State $\hat{y}_{train, i} \leftarrow VO(A(x_{train, i},P))$
                \State $g \leftarrow g + \nabla_{P} \ell_{train}(\hat{y}_{train, i}, y_{train, i})$
	        \EndFor
            \State $P \leftarrow P + \alpha \cdot \text{sign}(g)$
            \State $P \leftarrow clip(P,0,1)$
            \State \underline{\textbf{evaluate patch: }}
            \State $\text{Loss} \leftarrow 0$
	        \For{$i=1$ to $N_{eval}$}
                \State $\hat{y}_{eval, i} \leftarrow VO(A(x_{eval, i},P))$
                \State $\text{Loss} \leftarrow \text{Loss} + \ell_{eval}(\hat{y}_{eval, i}, y_{eval, i})$
	        \EndFor
	        \If{$\text{Loss} > \text{Loss}_\text{best}$}
                \State $P_\text{best} \leftarrow P$
                \State $\text{Loss}_\text{best} \leftarrow \text{Loss}$
	        \EndIf
    	\EndFor
		\State \textbf{return} $P_\text{best}$ 
	\end{algorithmic}
\end{algorithm}
\end{minipage}

==> visualizations/fig_synth_oos_small_patch.tex <==
\begin{figure*}
 \centering
    \begin{subfigure}{\linewidth}
        \includegraphics[width=0.483\linewidth]{figures/cumulative_RMS_to_distance_vs_trajectory_length__3sec_on_ring_r50m_60_frames_small_patch_out_of_sample_universal_attack_ablation.pdf}
        % \subcaption{A comparison of the produced deviation for our best performing universal attacks in out-of-sample attack scheme on synthetic data}
        \label{fig:synth_oos_small_patch}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \includegraphics[width=0.483\linewidth]{figures/cumulative_RMS_ratio_vs_trajectory_length__3sec_on_ring_r50m_60_frames_small_patch_out_of_sample_universal_attack_ablation.pdf}
        % \subcaption{A comparison of the produced deviation for our best performing universal attacks with different patch sizes in out-of-sample attack scheme on synthetic data}
        \label{fig:synth_oos_small_patch_ratio}
    \end{subfigure}
 \caption{
   Accumulated deviation in distance travelled from the ground-truth trajectories over out-of-sample cross-validation of the synthetic dataset as a function of the trajectory length. The patch is a $22.5[m]$ square and occupies an average FOV over the trajectories with range $8.3\%-12.6\%$, and mean $10.2\%$ area of the images. We show a deviation in distance travelled comparison of our universal attacks with smaller patch and the clean baseline (left) as well as the ratio of the deviation compared to the clean results (right). We present mean and standard deviation over the trajectories for each trajectory length.
 }
\label{fig:synth_oos_small_patch}
\end{figure*}

